Certifying unstability of Switched Systems using Sum of Squares Programming

The joint spectral radius (JSR) of a set of matrices characterizes the maximal asymptotic growth rate of an infinite product of matrices of the set. This quantity appears in a number of applications including the stability of switched and hybrid systems. A popular method used for the stability analysis of these systems searches for a Lyapunov function with convex optimization tools. We investigate dual formulations for this approach and leverage these dual programs for developing new analysis tools for the JSR. We show that the dual of this convex problem searches for the occupations measures of trajectories with high asymptotic growth rate. We both show how to generate a sequence of guaranteed high asymptotic growth rate and how to detect cases where we can provide lower bounds to the JSR. We deduce from it a new guarantee for the upper bound provided by the sum of squares lyapunov program. We end this paper with a method to reduce the computation of the JSR of low rank matrices to the computation of the constrained JSR of matrices of small dimension. All results of this paper are presented for the general case of constrained switched systems, that is, systems for which the switching signal is constrained by an automaton.

==> absdual.tex <==
%In this paper,
We show that the dual of this convex problem searches
for the \emph{occupations measures} of trajectories with high asymptotic growth
rate.
We both show how to generate a sequence of guaranteed high asymptotic growth rate and how to detect cases where we can provide lower bounds to the JSR.
%The moment relaxation of this problem is in fact the dual of the
%well known sum of squares optimization program for finding Lyapunov
%functions. Therefore, solving this program pair with a given candidate value
%for the JSR either returns Lyapunov functions certifying that the JSR
%is lower than this candidate value or returns the moments of relaxed
%occupation \emph{pseudo-measures}.
%We give a rounding procedure to extract high
%growth rate trajectories from these moments and provide a guarantee for
%this growth rate.
We deduce from it a new guarantee for the upper bound provided by the sum of squares lyapunov program.
%We can also detect that the
%JSR is larger than the candidate value by finding atomic measures that have
%the required moments.


==> absrank.tex <==
We end this paper with a method to reduce the computation of the JSR of
low rank matrices to the computation of the constrained JSR of matrices
of small dimension.

All results of this paper are presented for the general case of constrained switched systems,
that is, systems for which the switching signal is constrained by an automaton.
%For this reason, all results of this paper are generalized for constrained
%switched systems.


==> algotraj2meas.tex <==
\begin{algorithm}[!ht]
  \caption{Given %a family of measures $\nu_x$ parametrized by $x \in \Sn$ and
    a cycle $c$ of length $k$, builds a solution of \progref{dualinf} that is feasible for any $\gamlb \geq \jsrc$.}
    \label{algo:traj2meas}
    \begin{algorithmic}
      \STATE{Given a cyle $c = (\sigma_1, \ldots, \sigma_k)$ and a measure $\dirac{x}$ parametrized by $x \in \Sn$}
      \STATE{Pick \nodes{} $v_0, \ldots, v_{k-1},v_k=v_0 \in \Nodes$ such that $(v_{i-1}, v_i, \sigma_i) \in \Arcs$ for $i = 1, \ldots, k$}
      \STATE{Pick $x_0$ be such that $A_c x_0 = \lambda x_0$ with $|\lambda| = \rho(A_c)$ and $\enorm{x_0} = 1$}
      \FOR{$i = 1, 2, \ldots, k$}
      \STATE Set $x_i \leftarrow A_{\sigma_i} x_{i-1}$
      \STATE Set $\hat{x}_i \leftarrow x_i/\enorm{x_i}$
      \STATE Set $\alpha_i \leftarrow \enorm{x_i}/\jsrc^i$
      \ENDFOR
      \RETURN $(\,\mu_{uv\sigma} = \sum_{i=1,v_i = v}^k \alpha_i \dirac{\hat{x}_{i-1}} : (u,v,\sigma) \in \Arcs\,)$
    \end{algorithmic}
\end{algorithm}


==> continuous.tex <==
\section{Continuous case (WIP)}

Let $\mapd_\sigma$ be the linear map such that $\mapd_\sigma p(x) = [\grad(p(x))]^\Tr Ax$ for all $p(x) \in \R[x]_{\mathbf{2d}}$.
%Consider the scalar product such that $\la \pE, \mathcal{A}(p(x)) \ra$,
We define the adjoint map $\mapd_\sigma^*$,
the linear map such that $\la \mapd_\sigma^* \pE, p(x) \ra = \la \pE, \mapd_\sigma p(x) \ra$ for all $\pE \in (\R[x]_{\mathbf{2d}})^*$ and $p(x) \in \R[x]_{\mathbf{2d}}$.

The \emph{(worst case) Lyapunov exponent} $\lye$ is defined as
the infimum of the numbers $\lyea$ such that $\|x(t)\| \leq C\exp(\lyea t)$ for every trajectory.
That is,\footnote{More or less, just to write it as we like to see it}
\[ \exp(\lyea) = \lim_{t \to \infty} \sup_{\tau_1 + \cdots + \tau_k = t} \exp(A_{\sigma_k}\tau_k)\cdots\exp(A_{\sigma_1}\tau_1). \]

An upper bound $\lyesos \geq \lye$ is given by the following program.
\begin{myprog}[Primal]
  \label{prog:primalc}
  \begin{align}
    %\label{eq:sosprog}
    \notag
    \inf_{p(x) \in \Rh[x],\gamma \in \R} \gamma\\
    \label{eq:sosconsc1}
    p(x) & \text{ is SOS}\\
    \label{eq:sosconsc3}
    p(x) & \text{ is strictly positive}\\
    %\label{eq:soscons2}
    \notag
    \gamma^{2d} p(x) - \mapd_\sigma p(x) & \text{ is SOS} \quad \forall \sigma \in [m].
  \end{align}
\end{myprog}

The dual program is
\begin{myprog}[Dual]
  \label{prog:dualc}
  \begin{align}
    \notag
    \sup_{\pE_{\sigma} \in \Soshd, \gamma \in \R} \gamma\\
    \label{eq:dualconsexpc1}
    \sum_{\sigma \in [m]} \mapd_\sigma^* \pE_{\sigma} & \succeq \gamma^{2d} \sum_{\sigma \in [m]} \pE_{\sigma}, \forall v \in \Nodes,\\
    \label{eq:dualconsexpc3}
    \sum_{(u,v,\sigma) \in E} \pE_{uv\sigma}\Big[\sum_{i=1}^n x_i^{2d}\Big] & = 1.
    % FIXME the normalization equation (12) should probably be  E...[ (sum_i xi^2)^d ]  rather than  (sum_i x_i^2d).
    %       In a certain sense, it does not matter (since the purpose is to make the problem affine rather than homogeneous).
    %       However, this form is more symmetric, since now things are orthogonally invariant.
    %       It affects the numerical Example but we should do it later for the journal version and/or final submission.
  \end{align}
\end{myprog}

\todo{Give the algorithm and try to get bound with continuous $p$-radius, $1/\sqrt{m}$, $1/\sqrt{n}$}


==> invcone.tex <==
\section{Computing the $p$-radius}
\begin{mydef}[{\cite[Definition~2.5]{protasov1997generalized}}]
  Given two compact convex sets $\Cset_1,\Cset_2$ and $p \in [1,+\infty]$.
  The \emph{$p$-sum} of $\Cset_1$ and $\Cset_2$, denoted $\Cset_1 \psum \Cset_2$ is defined as the set
  \[ \Cset_1 \psum \Cset_2 = \setbuild{\alpha x + \beta y}{x \in \Cset_1, y \in \Cset_2, \|(\alpha,\beta)\|_q = 1} \]
  where $q \in [1,+\infty]$ is the conjugate of $p$, that is, $1/p + 1/q = 1$.
\end{mydef}

Note that for $p = 1$, this is the minkowski sum and for $p = \infty$, this is the convex hull.

Consider the following operator on convex sets defined in \cite{protasov1997generalized}
\[ \bar{A} \Cset = \bigoplus_{\sigma\in\{1,\ldots,m\}}^p A_k \Cset. \]

\begin{mytheo}[{\cite[Theorem~2]{protasov1997generalized}, \cite{rota1960note,jungers2009joint}}]
  \label{theo:invbody}
  If $\A = \{A_1, \ldots, A_m\}$ is an irreducible set of operators and $p \in [1, +\infty]$,
  then there exists a compact convex body $\Cset$ such that $\bar{A} \Cset = \lambda \Cset$ if and only if
  $\lambda = m^{\frac{1}{p}}\rho_p(\A)$ for $p < \infty$ and $\lambda = \rho(\A)$ for $p = \infty$.
\end{mytheo}

Consider the following generalization of \cite[Definition~2.1]{protasov2010joint}.
\begin{mydef}[{\cite[Definition~2.1]{protasov2010joint}}]
  For a compact set of matrices $\A$ with an invariant cone $\Kset$,
  we consider the value
  \[ \hat{\sigma}_\Kset = \inf \{\, \lambda \geq 0 \mid \exists v >_\Kset 0, \bar{A}v \leq_\Kset \lambda v \,\}. \]
\end{mydef}

We can generalize \cite[Lemma~2.4]{protasov2010joint} as follows.
\begin{mylem}
  For a compact set of matrices $\A$ with an invariant cone $\Kset$,
  we have
  \[ m^{\frac{1}{p}} \rho_p(\A) \leq \hat{\sigma}_\Kset. \]
  \begin{proof}
    Let $v >_\Kset 0$ and $\lambda \geq 0$ be such that $\bar{A}v \leq_\Kset \lambda v$.
    Consider the set $\Cset = (-v + \Kset) \cap (v - \Kset)$.
    We claim that $\bar{A} \Cset \subseteq \lambda \Cset$.
    Consider $v' \in \Cset$ and $w \in \Kset$ such that $v' = v - w$.
    We have $\bar{A}v' = \bar{A}v - \bar{A}w$.
    However, $\bar{A}w \subseteq \Kset$ by invariance of $K$ and $\bar{A}v \leq_\Kset \lambda v$ by assumption.
    Therefore $\bar{A}v' \subseteq \lambda(v-\Kset)$.
    The same reasoning can be used to prove that $\bar{A}v' \subseteq \lambda(-v+\Kset)$.
    Since $\Kset$ is solid, $\Cset$ is a compact convex body such that $\bar{A}\Cset \subseteq \lambda \Cset$.

    Consider now a compact convex body $\Cset'$ such that $\bar{A}\Cset' = \lambda' \Cset'$,
    by homogeneity and full-dimensionnality of $\Cset$, we can suppose that $\Cset' \subseteq \Cset$.
    By compactness of $\Cset$ and full-dimensionnality of $\Cset'$, there exist a finite constant $\beta > 1$
    such that $\Cset \subset \beta \Cset'$.
    If $\lambda' > \lambda$ then for $k > \log_{k'/k} \beta$, $\bar{A}^k \subset \bar{A}^k \Cset'$ which contradicts the fact that $\Cset' \subseteq \Cset$.
    This shows that $\lambda' \leq \lambda$.
    We can conclude by \theoref{invbody}.
  \end{proof}
\end{mylem}

\begin{mydef}[{\cite[Definition~2.5]{protasov2010joint}}]
  Given a cone $\Kset$, the value $\alpha(\Kset)$, $0 \leq \alpha \leq 1$,
  is the largest number such that for any convex compact set $\Cset \subseteq \Kset$,
  there exists $v \in \Cset$, for which $v \geq_\Kset \alpha \Cset$.
\end{mydef}

\begin{mydef}[{\cite[Theorem~2 f)]{protasov1997generalized}}]
  Given a compact convex set $\Cset \subseteq \R^d$,
  we define the \emph{$p$-norm} on $\Cset$, denoted $\|\Cset\|_p$ as follows
  \[ \|\Cset\|_p = \left[\sum_{i=1}^d [\delta^*(e_i|\Cset)]^p\right]^{\frac{1}{p}} \]
  where $e_i$ is the $i$th canonical vector or $\R^d$ and $\delta^*$ is the \emph{support function}; see \cite[Section~13]{rockafellar2015convex}.
\end{mydef}

\begin{mylem}[{\cite[Theorem~2 g)]{protasov1997generalized}}]
  Given finite integers $p \in [1,+\infty)$ and $k > 0$ and a compact convex set $\Cset$, the relation
  \[ \|\bar{A}^k \Cset\|_p = \left[\sum_{s \in \{1,\ldots,m\}^k} \|A_s \Cset\|_p^p\right]^{\frac{1}{p}}. \]
  holds.
\end{mylem}


==> svd.tex <==
\begin{lemma}
  \label{lem:svd}
  For any matrix $A \in \R^{n \times n}$ and symmetric positive semidefinite matrix $Q$,
  the following inequality holds
  \[ \rho(A^\Tr QA) \leq \rho(Q) \rho(A^\Tr A). \]
  \begin{proof}
    Since $Q$ is symmetric positive semidefinite,
    it has a Cholesky decomposition $Q = R^\Tr R$.
    Therefore we have
    %\begin{multline*}
    \begin{equation*}
      \rho(A^\Tr Q A) = \rho (A^\Tr R^\Tr R A)%\\
      = \|R A\|^2 \leq \|R\|^2 \|A\|^2 = \rho(Q) \rho(A^\Tr A).
    \end{equation*}
    %\end{multline*}
  \end{proof}
\end{lemma}

